Compositional Cyber-Physical Systems Modeling

Assuring the correct behavior of cyber-physical systems requires significant modeling effort, particularly during early stages of the engineering and design process when a system is not yet available for testing or verification of proper behavior. A primary motivation for `getting things right' in these early design stages is that altering the design is significantly less costly and more effective than when hardware and software have already been developed. Engineering cyber-physical systems requires the construction of several different types of models, each representing a different view, which include stakeholder requirements, system behavior, and the system architecture. Furthermore, each of these models can be represented at different levels of abstraction. Formal reasoning has improved the precision and expanded the available types of analysis in assuring correctness of requirements, behaviors, and architectures. However, each is usually modeled in distinct formalisms and corresponding tools. Currently, this disparity means that a system designer must manually check that the different models are in agreement. Manually editing and checking models is error prone, time consuming, and sensitive to any changes in the design of the models themselves. Wiring diagrams and related theory provide a means for formally organizing these different but related modeling views, resulting in a compositional modeling language for cyber-physical systems. Such a categorical language can make concrete the relationship between different model views, thereby managing complexity, allowing hierarchical decomposition of system models, and formally proving consistency between models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{125}
\providecommand{\publicationstatus}{David I. Spivak and Jamie Vicary (Eds.):\\
Applied Category Theory 2020 (ACT2020)\\
EPTCS 333, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.333.9}{10.4204/EPTCS.333.9}}
\pdfoutput=1


==> figures/ParallelCompo.tex <==


\begin{tikzpicture}[oriented WD, bbx = .5cm, bby =.8ex, bb min width=.5cm, bb port length=2pt, bb port sep=1]
\node[bb={2}{1}] (X) {$\mathtt{L}$};
\node[bb={2}{1}, below= 1.5 of X] (Y) {$\mathtt{C}$};
\node[bb={1}{1}, below=1.5 of Y] (Z) {$\mathtt{D}$};
\node at (0,-5.2) [draw,thick,dotted,minimum width=.7cm, minimum height=2cm] {};
\node[bb={2}{1}, fit={(X) (Y) (Z) ($(Z.south)-(0,5)$) ($(Z.east)+(1,0)$) ($(Z.west)-(1,0)$) ($(X.north)+(0,3)$)},gray] (C) {};
\draw[ar] (C_in1') to (X_in1);
\draw[ar] (C_in2') to (Y_in1);
\draw[ar] (X_out1)  to[in=0]  (.5,-16) to[out=180,in=0] (-.5,-16) to[out=180]  (Y_in2);
\draw[ar] (Y_out1) to[in=0]  (.5,-15) to[out=180,in=0] (-.5,-15) to[out=180] (Z_in1);
\draw[ar] (Z_out1) to (C_out1');
\draw[ar] (Z_out1) to[in=0]  (.5,-14) to[out=180,in=0] (-.5,-14) to[out=180] (X_in2);
\draw[label]
node[above right=.2 of X_out1] {\tiny x}
node[above right=.2 of Y_out1] {\tiny y}
node[below right=.45 of Z_out1] {\tiny z}
node[above left=.2 of X_in1] {\tiny w}
node[above left=.2 of Y_in1] {\tiny v}
node[above right=2 and 1 of X_out1] {$\mathtt{U}$}
node (text) [right=2.5 of Y,rectangle,align=left]
{\scriptsize$ f_\inp\colon\overbrace{\mathbb{R}^3}^{(L\otimes C\otimes D)_\out}\times \overbrace{\mathbb{R}^2}^{U_\inp}\to\overbrace{\mathbb{R}^5}^{(L\otimes C\otimes D)_\inp} \textrm{by } (x,y,z,w,v)\mapsto (w,z,v,x,y)$\\
\scriptsize$f_\out\colon\underbrace{\mathbb{R}^3}_{(L\otimes C\otimes D)_\out}\to\underbrace{\mathbb{R}}_{U_\out}\phantom{ABCDEAAA} \textrm{by } (x,y,z)\mapsto z$};
 \end{tikzpicture}


==> figures/UAVwiringdiagram.tex <==


\begin{tikzpicture}[oriented WD, bbx = .5cm, bby =.8ex, bb min width=.5cm, bb port length=2pt, bb port sep=1]
\node[bb={2}{1}] (L) {$\mathtt{L}$};
\node[bb={2}{1}, above right= 0.01cm and 1cm of L] (C) {$\mathtt{C}$};
\node[bb={1}{1}, below right= 0.01cm and 1cm of C] (D) {$\mathtt{D}$};
\node[bb={2}{1}, fit={($(L.west)-(1,0)$) ($(D.east)+(1,0)$) ($(L.south)-(0,5)$) ($(C.north)+(0,3)$)},gray] (A) {};
 \draw[ar] (A_in2') to (L_in1);
  \draw[ar] (A_in1') to (C_in1);
 \draw[ar] (L_out1) to (C_in2);
 \draw[ar] (C_out1) to (D_in1);
 \draw[ar] (D_out1) to (A_out1');
  \draw[ar] (D_out1) .. controls ($ (D_out1) +(3.5,-9)$) and ($ (L_in2) -(2,9)$) .. (L_in2);
\draw[label]
node[left=.1 of A_in1] {$\mathbb{R}$}
node[left=.1 of A_in2]{$\mathbb{R}$}
node[right=.1 of A_out1]{$\mathbb{R}$}
node[above right= of L_out1]{$\mathbb{R}$}
node[above right= of C_out1]{$\mathbb{R}$}
node[above right= .5 and 4 of C]{$\mathtt{U}$};
 \end{tikzpicture}


==> figures/implementation.tex <==

\begin{tikzpicture}[oriented WD, bbx = .5cm, bby =.8ex, bb min width=.5cm, bb port length=2pt, bb port sep=1]
\node[bb={2}{1}] (P) {$\mathtt{P}_1$};
\node[bb={1}{1},above left=of P] (I) {$\mathtt{I}_1$};
\node[bb={1}{1},below left=of P] (J) {$\mathtt{I}_2$};
\node[bb={2}{1},inner sep=.1in,fit={(J)(I)(P)},red] (L) {};
\node[bb={2}{1}, above right= 0.8cm and 1.5cm of L] (Q) {$\mathtt{P}_2$};
\node[bb={1}{1},right= of Q] (V) {$\mathtt{V}$};
\node[bb={2}{1}, inner sep=.1in,fit={(Q)(V)},blue] (C) {};
\node[bb={1}{1}, below right=0.8cm and 1.5cm of C] (X) {$\mathtt{X}$};
\node[bb={1}{1}, below=.01cm of X] (Y) {$\mathtt{Y}$};
\node[bb={1}{1}, below=.01cm of Y] (Z) {$\mathtt{Z}$};
\node[bb={1}{1}, below=.01cm of Z] (U) {$\mathtt{W}$};
\node[bb={4}{1}, right=7cm of P] (F) {$\mathtt{F}$};
\node[bb={1}{1}, fit={(X)(U)(F)},brown] (D) {};
\node[bb={2}{1}, fit={($(L.west)-(1,0)$) ($(D.east)+(1,0)$) ($(L.south)-(0,15)$) ($(C.north)+(0,3)$)},gray] (A) {};
\draw[ar] (L_in1') to (I_in1);
\draw[ar] (L_in2') to (J_in1);
\draw[ar] (I_out1) to (P_in1);
\draw[ar] (J_out1) to (P_in2);
\draw[ar] (P_out1) to (L_out1');
 \draw[ar] (A_in2') to (L_in1);
  \draw[ar] (A_in1') to (C_in1);
 \draw[ar] (L_out1) to (C_in2);
 \draw[ar] (C_out1) to (D_in1);
 \draw[ar] (V_out1) to node[above,blue]{$\mathtt{C}$} (C_out1');
 \draw[ar] (D_out1) to (A_out1');
\draw[ar] (C_in1') to (Q_in1);
\draw[ar] (C_in2') to (Q_in2);
\draw[ar] (Q_out1) to (V_in1);
\draw[ar] (D_in1') to (X_in1);
\draw[ar] (D_in1') to (Y_in1);
\draw[ar] (D_in1') to (Z_in1);
\draw[ar] (D_in1') to (U_in1);
\draw[ar] (X_out1) to (F_in1);
\draw[ar] (Y_out1) to (F_in2);
\draw[ar] (Z_out1) to (F_in3);
\draw[ar] (U_out1) to (F_in4);
\draw[ar] (F_out1) to (D_out1');
\draw[ar] (D_out1) .. controls ($ (D_out1) +(4,-25)$) and ($ (L_in2) -(4,25)$) .. (L_in2);
\node[above right= .5 and 7 of C]{$\mathtt{UAV}$};
\node[right=1cm of I,red]{$\mathtt{L}$};
\node[right=1.3cm of X,brown]{$\mathtt{D}$};
 \end{tikzpicture}


==> figures/system_function.tex <==

\begin{tikzpicture}[oriented WD, bbx = .5cm, bby =.8ex, bb min width=.5cm, bb port length=2pt, bb port sep=1]
\node[bb={2}{1}] (L) {\begin{tabular}{c}
     sensor  \\
     $\mathtt{L}$
\end{tabular}};
\node[bb={2}{1}, above right= 0.01cm and 1cm of L] (C) {
\begin{tabular}{c}
     controller\\ $\mathtt{C}$
\end{tabular}};
\node[bb={1}{1}, below right= 0.01cm and 1cm of C] (D) { \begin{tabular}{c}
     dynamics\\ $\mathtt{D}$
\end{tabular}};
\node[bb={2}{1}, fit={($(L.west)-(1,0)$) ($(D.east)+(1,0)$) ($(L.south)-(0,5)$) ($(C.north)+(0,3)$)},gray] (A) {};
 \draw[ar] (A_in2') to (L_in1);
  \draw[ar] (A_in1') to (C_in1);
 \draw[ar] (L_out1) to (C_in2);
 \draw[ar] (C_out1) to (D_in1);
 \draw[ar] (D_out1) to (A_out1');
  \draw[ar] (D_out1) .. controls ($ (D_out1) +(3.5,-11)$) and ($ (L_in2) -(2,11)$) .. (L_in2);
\node (text) [below=15 of C,rectangle,align=left]
{$ f_\inp\colon\mathbb{R}^3\times\mathbb{R}^2\to\mathbb{R}^5,\; (s',c,s,e,d)\mapsto(e,s,d,s',c)$ \\
$ f_\out\colon\mathbb{R}^3\to \mathbb{R},\;(s',c,s)\mapsto s$};
\draw[label]
node[left=.1 of A_in1] {$\mathbb{R}$}
node[left=.1 of A_in2]{$\mathbb{R}$}
node[right=.1 of A_out1]{$\mathbb{R}$}
node[above right= 4 and .3 of L_out1]{$\mathbb{R}$}
node[below right= 1 and .8 of C_out1]{$\mathbb{R}$}
node[above right= of A_in1']{$d$}
node[above right= of A_in2']{$e$}
node[above right= of L_out1]{$s'$}
node[above right= of C_out1]{$c$}
node[above right= of D_out1]{$s$}
node[above right= .5 and 6 of C]{$\mathtt{UAV}$};
 \end{tikzpicture}

